Supporting Post-disaster Recovery with Agent-based Modeling in Multilayer Socio-physical Networks

The examination of post-disaster recovery (PDR) in a socio-physical system enables us to elucidate the complex relationships between humans and infrastructures. Although existing studies have identified many patterns in the PDR process, they fall short of describing how individual recoveries contribute to the overall recovery of the system. To enhance the understanding of individual return behavior and the recovery of point-of-interests (POIs), we propose an agent-based model (ABM), called PostDisasterSim. We apply the model to analyze the recovery of five counties in Texas following Hurricane Harvey in 2017. Specifically, we construct a three-layer network comprising the human layer, the social infrastructure layer, and the physical infrastructure layer, using mobile phone location data and POI data. Based on prior studies and a household survey, we develop the ABM to simulate how evacuated individuals return to their homes, and social and physical infrastructures recover. By implementing the ABM, we unveil the heterogeneity in recovery dynamics in terms of agent types, housing types, household income levels, and geographical locations. Moreover, simulation results across nine scenarios quantitatively demonstrate the positive effects of social and physical infrastructure improvement plans. This study can assist disaster scientists in uncovering nuanced recovery patterns and policymakers in translating policies like resource allocation into practice.

==> road_segment_network.tex <==
\section{Road Segment Network}

Based on the critical relative speed $\rho_{c}$ from the percolation road network curves, we construct the road segment network (RSN), on which we will apply the network partitioning algorithm. In network science, network partitioning aims to divide the whole network into subnetworks that are non-overlapping \cite{newman2018networks}. The fundamental principle of network partitioning is that the link connections within the subnetwork are strong while the link connections between two subnetworks are weak. Existing urban road network partitioning algorithms such as Ji and Geroliminis \cite{ji2012spatial}, An et al. \cite{an2017network} also followed this principle. They defined the link connectivity between road segments $i$ and $j$ as a function that was inversely proportional to the gap of road segment density $k_i$ and $k_j$, which was $|k_i-k_j|$. Under this definition, a strong link connection within a subnetwork is equivalent to a homogeneous distribution of link density values, which naturally matches the requirement of a well-defined MFD.

Recall that we decide to utilize the road segment data and the percolation road network curve to feed the network partitioning algorithm in this study. We set our partitioning objective as: road segments within one subnetwork have a significant contribution on critical relative speed $\rho_{c}$ (i.e., the connectivity-based congestion index). The practical understanding of this objective is that different subnetworks in a partitioning outcome may be managed separately in the real world (i.e., different control periods, management policies, and traffic police) so that we seek to put two links in the same subnetwork if they have a large joint contribution on regional traffic. Based on our network partitioning objective and the aforementioned fundamental principle of network partitioning, we therefore define the connectivity strength of road segments $i$ and $j$ as their joint contribution on $\rho_{c}$ for their regional network. 

We provide the rigorous definition of the RSN now. The RSN is a dual representation $G^{d}(V^{d}, A^{d})$ \cite{porta2006network,zhan2017dynamics} of the road network whose node set $V^{d}$ and link set $A^{d}$ denote the road segments and the adjacency relationships between road segments, respectively. Assume that $V^{d}$ consists of $m$ road segments:
\begin{equation}
    V^{d}=\{v^{d}_{1},v^{d}_{2},...,v^{d}_{m}\}.
\end{equation}
For any two nodes $v^{d}_{i}$, $v^{d}_{j}$ $(1\leq i< j\leq m)$, if road segments $v^{d}_{i}$ and $v^{d}_{j}$ do not share a same intersection, we define the link weights as:
\begin{equation}
    a^{d}_{ij}=a^{d}_{ji}=0.
\end{equation}
Otherwise, we use the $\rho_{c}$ to define the link weight as follows. Assume that road segments $v^{d}_{i}$ and $v^{d}_{j}$ share one common intersection $u(i,j)$. We refer to the square region centering at the intersection $u(i,j)$ with a side length of $r$ as the region $\Gamma_{r}(i,j)$. Notice that we know the longitude and latitude of all road segments and intersections, so that we are able to select all road segments and intersections belonging to the region $\Gamma_{r}(i,j)$, and then define a network $G^{r,i,j}$ using these road segments and intersections. For $G^{r,i,j}$, we generate the percolation curve $\nu(\rho) - \rho$, which is a non-increasing function:
\begin{equation}
   \nu(\rho|r,i,j,r_{i}(t),r_{j}(t)): [0,1] \rightarrow [0,1], 
\end{equation}
\begin{equation}
   \rho \mapsto \nu(\rho|r,i,j,r_{i}(t),r_{j}(t)) = \frac{|LCC(G^{r,i,j}_{u}(\rho))|}{|G^{r,i,j}|}.
\end{equation}
Recall that $r_{i}(t)$ and $r_{j}(t)$ are relative road segment speeds (please see equation (\ref{relative speed})). We define the critical relative speed $\rho_{c}(r,i,j,r_{i}(t),r_{j}(t))$ for the network $G^{r,i,j}$ as
\begin{equation}
    \rho_{c}(r,i,j,r_{i}(t),r_{j}(t)) = argmax_{\rho\in [0,1]}\frac{-\partial \nu(\rho |r,i,j,r_{i}(t),r_{j}(t))}{\partial \rho}.
    \label{rho_equation}
\end{equation}
Finally, we define the link weights in $G^{d}(V^{d}, A^{d})$ as 
\begin{equation}
    a_{ij}^{d}=a_{ji}^{d}=\rho_{c}(r,i,j,r'_{i}(t),r'_{j}(t))-\rho_{c}(r,i,j,r_{i}(t),r_{j}(t)),
    \label{define_connection}
\end{equation}
where $r'_{i}(t),r'_{j}(t)$ represent the average relative road segment speed after improvements. In practice, we can set $r'_{i}(t)=r_{i}(t)(1+\delta) , r'_{j}(t)=r_{j}(t)(1+\delta)$ where $\delta$ is a hypothetical relative road segment speed increase ratio (i.e., $\delta$=0.05, which was used in Li et al. \cite{li2015percolation}), or set the new relative speed as unity (i.e., $r'_{i}(t)=r'_{j}(t)=1$, which was used in Hamedmoghadam et al. \cite{hamedmoghadam2021percolation}).

We clarify the reasons for the aforementioned definition of $a_{ij}^{d}$. First, for non-adjacent road segments $v_i^{d}$ and $v_j^{d}$, the link weights $a_{ij}^{d}$ and $a_{ji}^{d}$ are set to be zero because $v_i^{d}$ and $v_j^{d}$ are not directly joined. Second, for adjacent road segments $v_i^{d}$ and $v_j^{d}$ within the area $\Gamma_{r}(i,j)$, $\rho_{c}(r,i,j,r_{i}(t),r_{j}(t))$ is the maximal relative speed $\rho$ where links with relative speed larger than $\rho$ maintain the global connectivity, so that it measures the connectivity of good-traffic-condition roads. Note that the connectivity of these roads serves as an indicator representing network-level traffic and connecting personal mobility experience. We therefore set our network partitioning objective as to increase the $\rho_{c}$, and accordingly, define the link weight $a_{ij}^{d}$ and $a_{ji}^{d}$ as the increment of $\rho_{c}$ by  $v_i^{d}$ and $v_j^{d}$. Hence, based on our objective and the principle of network partitioning, we seek to obtain the partitioning solution whose subnetworks have suitable structures to be improved regarding regional connectivity $\rho_{c}$. 



